Edge Conditional Node Update Graph Neural Network for Multi-variate Time Series Anomaly Detection

With the rapid advancement in cyber-physical systems, the increasing number of sensors has significantly complicated manual monitoring of system states. Consequently, graph-based time-series anomaly detection methods have gained attention due to their ability to explicitly represent relationships between sensors. However, these methods often apply a uniform source node representation across all connected target nodes, even when updating different target node representations. Moreover, the graph attention mechanism, commonly used to infer unknown graph structures, could constrain the diversity of source node representations. In this paper, we introduce the Edge Conditional Node-update Graph Neural Network (ECNU-GNN). Our model, equipped with an edge conditional node update module, dynamically transforms source node representations based on connected edges to represent target nodes aptly. We validate performance on three real-world datasets: SWaT, WADI, and PSM. Our model demonstrates 5.4%, 12.4%, and 6.0% higher performance, respectively, compared to best F1 baseline models.

==> 4.7.1.table-1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[htb!]
\caption{Results of ablation study for effects of node embedding vectors}
\label{table:abl_cond}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|ccc|ccc|ccc|}
\hline
\multirow{2}{*}{\textbf{Methods}} & \multicolumn{3}{c|}{\textbf{SWaT}}                                                           & \multicolumn{3}{c|}{\textbf{WADI}}                                                           & \multicolumn{3}{c|}{\textbf{PSM}}                                                            \\ \cline{2-10} 
                                  & \multicolumn{1}{c|}{\textbf{F1}} & \multicolumn{1}{c|}{\textbf{Recall}} & \textbf{Precision} & \multicolumn{1}{c|}{\textbf{F1}} & \multicolumn{1}{c|}{\textbf{Recall}} & \textbf{Precision} & \multicolumn{1}{c|}{\textbf{F1}} & \multicolumn{1}{c|}{\textbf{Recall}} & \textbf{Precision} \\ \hline
\textbf{Original}                 & \multicolumn{1}{c|}{0.8541}           & \multicolumn{1}{c|}{0.7593}               & 0.9761                  & \multicolumn{1}{c|}{0.6405}           & \multicolumn{1}{c|}{0.5257}               & 0.8207                  & \multicolumn{1}{c|}{0.6179}           & \multicolumn{1}{c|}{0.6986}               & 0.5339                  \\ \hline
\textbf{-Target(T)}               & \multicolumn{1}{c|}{0.8213}          & \multicolumn{1}{c|}{0.7470}              & 0.9122                 & \multicolumn{1}{c|}{0.5716}          & \multicolumn{1}{c|}{0.5059}              & 0.6577                 & \multicolumn{1}{c|}{0.6093}          & \multicolumn{1}{c|}{0.7053}              & 0.5364                 \\ \hline
\textbf{-Source(S)}               & \multicolumn{1}{c|}{0.7967}          & \multicolumn{1}{c|}{0.6676}              & 0.9881                 & \multicolumn{1}{c|}{0.4508}          & \multicolumn{1}{c|}{0.3218}              & 0.7541                 & \multicolumn{1}{c|}{0.6090}          & \multicolumn{1}{c|}{0.6364}              & 0.5839                 \\ \hline
\textbf{-Readout(R)}              & \multicolumn{1}{c|}{0.8497}          & \multicolumn{1}{c|}{0.7468}              & 0.9858                 & \multicolumn{1}{c|}{0.5760}          & \multicolumn{1}{c|}{0.4238}              & 0.9011                 & \multicolumn{1}{c|}{0.5955}          & \multicolumn{1}{c|}{0.6705}              & 0.5356                 \\ \hline
\textbf{-T,R}                     & \multicolumn{1}{c|}{0.8336}          & \multicolumn{1}{c|}{0.7240}              & 0.9825                 & \multicolumn{1}{c|}{0.4955}          & \multicolumn{1}{c|}{0.4376}              & 0.5689                 & \multicolumn{1}{c|}{0.6036}          & \multicolumn{1}{c|}{0.6471}              & 0.5657                 \\ \hline
\textbf{-S,R}                     & \multicolumn{1}{c|}{0.7992}          & \multicolumn{1}{c|}{0.7186}              & 0.8999                 & \multicolumn{1}{c|}{0.4591}          & \multicolumn{1}{c|}{0.3277}              & 0.7680                 & \multicolumn{1}{c|}{0.6040}          & \multicolumn{1}{c|}{0.6718}              & 0.5485                 \\ \hline
\textbf{-S,T}                     & \multicolumn{1}{c|}{0.7885}          & \multicolumn{1}{c|}{0.6769}              & 0.9446                 & \multicolumn{1}{c|}{0.4676}          & \multicolumn{1}{c|}{0.3129}              & 0.9159                 & \multicolumn{1}{c|}{0.6019}          & \multicolumn{1}{c|}{0.6777}              & 0.5414                 \\ \hline
\end{tabular}%
}
\end{table}

==> 4.7.2.fig.tex <==

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{swat_wh_attn_mean.png}
    \caption{Similarity between node representations with graph attention}
    \label{fig:swat_wh_attn_mean_rep}
\end{figure}

\begin{figure}
\centering
    \includegraphics[width=\textwidth]{swat_wo_attn_mean.png}
    \caption{Similarity between node representations without graph attention}
    \label{fig:swat_wo_attn_mean_rep}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{swat_wh_attn_mean_before.png}
    \caption{Similarity between source and target representations before updating target nodes with graph attention}
    \label{fig:swat_wh_attn_mean_before}
\end{figure}

\begin{figure}
\centering
    \includegraphics[width=\textwidth]{swat_wo_attn_mean_before.png}
    \caption{Similarity between source and target representations before updating target nodes without graph attention}
    \label{fig:swat_wo_attn_mean_before}

\end{figure}



==> 4.7.2.table_origin.tex <==

\begin{table}[htb!]
\caption{Similarity comparison results for each dataset}
\label{table:attn_result}
\resizebox{\textwidth}{!}{
%\centering
\begin{tabular}{|c|c|c|cc|cc|}
\hline
\textbf{Dataset}               & \textbf{Model}      & \textbf{F1} & \textbf{Train} $sim_{\textit{rep}}$ & \textbf{Val} $sim_{\textit{rep}}$ & {\textbf{Train} $sim_{\textit{trf}}$} & \textbf{Val} $sim_{\textit{trf}}$ \\ \hline
\multirow{2}{*}{\textbf{SWaT}} & \textbf{Origin}     & 0.8541      & 0.6457                      & 0.6516                    & 0.5867                                           & 0.5899                    \\
                               & \textbf{+Attention} & 0.8257      & 0.9248                      & 0.9244                    & 0.7832                                           & 0.7810                    \\ \hline
\multirow{2}{*}{\textbf{WADI}} & \textbf{Origin}     & 0.6405      & 0.4664                      & 0.4754                    & 0.2590                                           & 0.2584                    \\
                               & \textbf{+Attention} & 0.5134      & 0.8446                      & 0.8654                    & 0.5985                                           & 0.6611                    \\ \hline
\multirow{2}{*}{\textbf{PSM}} & \textbf{Origin}     & 0.6405      & 0.4664                      & 0.4754                    & 0.2590                                           & 0.2584                    \\
                               & \textbf{+Attention} & 0.5134      & 0.8446                      & 0.8654                    & 0.5985                                           & 0.6611                    \\ \hline                               
\end{tabular}}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% new table origin
\begin{table}[]
\caption{Similarity comparison results for each dataset}
\label{table:attn_result}
\resizebox{\textwidth}{!}{
%\centering
\begin{tabular}{|c|c|c|c|cc|}
\hline
\textbf{Dataset}               & \textbf{Model}      & \textbf{F1} & $sim_{Total}$& $sim^{t}$ Mean & $sim^{t}$ Std  \\ \hline
\multirow{3}{*}{\textbf{SWaT}} & \textbf{Origin}     & 0.8541      & 0.8095                      & 0.5120&0.2351                                        \\
                               & \textbf{+Vanilla} & 0.8257      & 0.9911                      & 0.8857&0.0771                            \\ 
                               & \textbf{+Node-wise} & 0.7939      & 0.9754                      & 0.8088&0.1000                            \\ \hline
\multirow{3}{*}{\textbf{WADI}} & \textbf{Origin}     & 0.6405      & 0.3937                      & 0.1940&0.2686                    \\
                               & \textbf{+Vanilla} & 0.5134      & 0.6826                      & 0.6647&0.1389                    \\
                               & \textbf{+Node-wise} & 0.5678      & 0.5316                      & 0.6361 &0.2357                            \\ \hline
\multirow{3}{*}{\textbf{PSM}} & \textbf{Origin}     & 0.6179      & 0.6655                      & 0.2247&0.2539                    \\
                             & \textbf{+Vanilla} & 0.6140      & 0.5347                      & 0.6285&0.1878                \\
                            & \textbf{+Node-wise} & 0.5828      & 0.6707                      & 0.6257&0.1457                 \\
                            \hline                               
\end{tabular}}
\end{table}
